Learning Heuristics over Large Graphs via Deep Reinforcement Learning

There has been an increased interest in discovering heuristics for combinatorial problems on graphs through machine learning. While existing techniques have primarily focused on obtaining high-quality solutions, scalability to billion-sized graphs has not been adequately addressed. In addition, the impact of budget-constraint, which is necessary for many practical scenarios, remains to be studied. In this paper, we propose a framework called GCOMB to bridge these gaps. GCOMB trains a Graph Convolutional Network (GCN) using a novel probabilistic greedy mechanism to predict the quality of a node. To further facilitate the combinatorial nature of the problem, GCOMB utilizes a Q-learning framework, which is made efficient through importance sampling. We perform extensive experiments on real graphs to benchmark the efficiency and efficacy of GCOMB. Our results establish that GCOMB is 100 times faster and marginally better in quality than state-of-the-art algorithms for learning combinatorial algorithms. Additionally, a case-study on the practical combinatorial problem of Influence Maximization (IM) shows GCOMB is 150 times faster than the specialized IM algorithm IMM with similar quality.

==> 5_1_application.tex <==
\subsection{Application: Temporal Networks}
The primary motivation behind \gc is the observation that many real-world networks change with time although the underlying model remains the same. Temporal networks is one such example. In this section, we show that \gc is ideally suited for this scenario. Specifically, we establish that if \gc is trained on today's network snapshot, it can predict solutions to combinatorial optimization problems on future network snapshots accurately. 
%We show an application of our method, GCOMB on temporal networks. As a temporal network does not vary significantly over time, the structural distribution remains same. We aim to evaluate applicability of our method on these networks. The goal is to show that GCOMB will predict the solution set correctly on graphs over different time snapshots
%while being trained on a few of them.

To demonstrate \gc's predictive power on temporal networks, we considered a question-answer platform, namely the sx-mathoverflow (SM) dataset (Table \ref{table:data_description}). The nodes correspond to users and an edge at a time $t$ depicts an interaction between two users (Ex: answering or commenting to questions) at time $t$. The data consists of interaction over a span of $2350$ days.
To generate train and test graphs, we split the span of 2350 days into 55 equal spans (around 42 days) and consider all interactions (edges) inside a span for the corresponding graph. We denote these as $\mathcal{G}= \{G_i| i=1,2,\cdots, 55\}$. We use multiple interactions between a pair of users as the weight of the edge between them. The edge-weight is used as a feature (activity of an user) in the GCN. For training, we pick the graphs $G_{0},\cdots,G_{4}$ and $G_{21},\cdots,G_{26}$ for the MCP and MVC problems respectively and then test on all of the remaining graphs. 

Figure \ref{fig:temporal} presents the performance of \gc. As visible, the quality of \gc's solutions sets are almost identical to GR across all test graphs. %Besides that, our method shows similar trend as in greedy algorithm and that shows that for same distribution, GCOMB can learn and predict greedy heuristic efficiently. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% temporal applications
\begin{figure}[t]
%\vspace{-5mm}
    \centering
    \subfloat[MVC]{\includegraphics[width=0.24\textwidth]{Figures/temporal/mvc_dynamic.pdf}\label{fig:temporal_mvc}} 
    \subfloat[MCP]{\includegraphics[width=0.24\textwidth]{Figures/temporal/msc_dynamic.pdf}\label{fig:temporal_msc}}
    % \vspace{-0.10in}
    \caption{\textbf{Quality of the solution sets produced by \gc and GR on temporal networks.} 
    \label{fig:temporal}}
    % \vspace{-0.10in}
\end{figure}

==> 5_2_IMM.tex <==
\begin{figure*}[t]
	\centering
%\vspace{-0.20in}
\subfloat[Scalability]{
\label{fig:time_nips}
\includegraphics[width=1.27in]{Figures/time_nips.pdf}}
\subfloat[Quality]{
\label{fig:quality_nips}
\includegraphics[width=1.30in]{Figures/quality_nips.pdf}}
\subfloat[Speed-up in YouTube]{
	\label{fig:speedup_yt}
	\includegraphics[width=1.20in]{Figures/speedup_yt.pdf}}
\subfloat[Speed-up in Stack]{
	\label{fig:speedup_st}
	\includegraphics[width=1.20in]{Figures/speedup_st.pdf}}
	\caption{ Comparison of (a) scalability and (b) quality on subgraphs extracted from YT (Table~\ref{table:data_description}) at budget=$20$. (c-d) Speed-up achieved by \gc over IMM in YT and Stack. }
% \vspace{-0.20in}
\end{figure*}

% \vspace{-0.10in}
\subsection{Performance on Influence Maximization}
\label{sec:im}
% \vspace{-0.10in}

Influence Maximization (IM) is the hardest of the three combinatorial problems since estimating the spread of a node is \#P-hard \cite{kempe2003maximizing}. %Owing to this reason, even Greedy is exorbitantly slow. %The state of the art in this space is IMM \cite{benchmarking,imm}.%e%hus, we train \gc using the solution sets of IMM.  
 %We compare the performance of \gc with IMM on five of the largest real datasets from Table~\ref{table:data_description}. 
% We skip \gt since as discussed in \S~\ref{sec:intro}, \gt is significantly inferior in both quality and efficiency. 
 

%\vspace{-0.05in}
\textbf{Edge weights: } %Edge weights denote the influence of a connection in a social network. 
We assign edge weights that denote the influence of a connection using the two popular models \cite{benchmarking}: \textbf{(1) Constant (CO:)} All edge weights are set to $0.1$, \textbf{(2) Tri-valency (TV): } Edge weights are sampled randomly from the set $\{0.1, 0.01, 0.001\}$. In addition, we also employ a third \textbf{(3) Learned (LND)} model, where we \emph{learn} the influence probabilities from the action logs of users. This is only applicable to the Stack data which contain \emph{action logs} from $8/2008$ to $3/2016$. %Among our datasets, only Stack contains \emph{action logs} from $8/2008$ to $3/2016$, and thus this model is applicable only in Stack. %Stack is a communication forum where users correspond to nodes and each edge corresponds to an action. Edges are annotated with timestamps denoting when the action took place. An action corresponds to user $u$ answering $v$'s question, $u$ commenting on $v$'s question, or $u$ commenting on $v$'s answer. 
We define the influence of $u$ on $v$ as the probability of $v$ interacting with $u$'s content at least once in a month. 

%, \textbf{(3) WC: } All incoming neighbors of node $v$ influence $v$ with equal probability, i.e., $W(u,v)=\frac{1}{|In(v)|}$ where $In(v)$ is the set of incoming neighbors of $v$. 

\textbf{Train-Validation-Test split: } In all of the subsequent experiments, for CO and TV edge weight models, we train and validate on a subgraph sampled out of YT by randomly selecting $30\%$ of the edges ($50\%$  of the subset is used for training and $50\%$ for validation). For LND edge weight models, we train and validate on the subgraph induced by the $30\%$ of the earliest edges from Stack in terms of temporal order. While testing, on YT and Stack, we use the network formed by the remaining $70\%$ of the edges that are not used for training. On other datasets, we use the entire network for testing since neither those datasets nor their subsets are used for training purposes.  %Similarly in Stack, while evaluating the LND edge weights model, we only use the edges that are not used for training. 
%In general, we always ensure that the test set is completely unseen. %Due to the slowness of Greedy, we use IMM\cite{imm} to compute spread of a node while training \gc.
\begin{comment}
% \vspace{-0.05in}
\subsubsection{Performance of \gt} Fig.~\ref{fig:motivation} shows that \gt is more than $1000$ times slower than \gc. In addition, the quality of \gt is also inferior. In Fig.~\ref{fig:motivation}, we use the TV edge weight model at budget $b=20$. Sec.~\ref{sec:relatedwork} discusses in detail both the non-scalability of \gt and how the quality suffers when the combinatorial problem cannot be easily mapped from the Maximal
Independent Set problem. As a result, we use the IMM algorithm \cite{imm} as our primary baseline in the IM problem.
\end{comment}
% stems from two factors: first, GCN is called repeatedly and second, TreeSearch is extremely slow as computing the marginal gain is \#P-hard. In contrast, \gc calls GCN only once and the marginal gain of adding a node is predicted whose complexity is linear to the embedding dimension ($256$). This non-scalability of \gt limits us from benchmarking it on larger datasets. In subsequent experiments for IM, we thus compare the performance of \gc against IMM, which is specifically built for the IM problem. 

%\subsubsection{Non-scalability of \gt} In the IM problem, the quality of \gt suffers due to three main reasons. \textbf{(1)} In typical problems like vertex cover or set cover, the coverage of a node is deterministic. In IM, the coverage, or spread, is an \emph{expectation}. To estimate this expectation well, we need to perform a large number of MC simulations ($1000$ or more\cite{benchmarking}). However, in TreeSearch, where we search the overlap among expected spread of various nodes, we are limited to a small number ($50$) due to scalability issues already pointed out. Hence, the quality suffers. \gc does not suffer since it simply predicts the spread and resultant marginal gains. \textbf{(2)} The GCN architectures are different. While we use GraphSage\cite{hamilton2017inductive}, \gt uses \cite{gcn}. Furthermore, \gt does not use any node features. \textbf{(3)}. \gt uses cross-entropy loss to predict the answer set of only a specific budget. Thus, if the input budget is different, the quality may suffer. In contrast, \gc uses a budget-independent scoring function (Eq.~\ref{eq:score}), which is trained using mean squared error. In Fig.~\ref{fig:motivation}, the training and testing budget for \gt is kept the same.
%TreeSearch component works as follows: First, in IM, the quality of a node, that is expected spread, is computed through a large number of MC simulations (1000 or more). In TreeSearch, we performed 50 MC simulations since anything more further hampers the scalability. 

\textbf{\gc vs.\gt: }Fig.~\ref{fig:time_nips} and Fig.~\ref{fig:quality_nips} compare the running time and quality in IM on YT. While \gt consumes $\approx 3$ hours on the $70\%$ sub-network, \gc finishes in $5$ seconds. The quality of \gc is also significantly better since IM is not easily mappable to the MIS problem, for which \gt is built. %As was discussed in details in \S~\ref{sec:relatedwork}, 

 \textbf{Billion-sized networks:}  IMM crashes on both the billion-sized datasets of TW and FS, as well as Orkut. Unsurprisingly, similar results have been reported in \cite{benchmarking}. IMM strategically samples a subgraph of the entire network based on the edge weights. On this sampled subgraph, it estimates the influence of a node using \emph{reverse reachability sets}. 
On large networks, the sample size exceeds the RAM capacity of 256GB. Hence, it crashes.
 In contrast, \gc finishes within minutes for smaller budgets ($b<30$) and within $100$ minutes on larger budgets of $100$ and $200$ (Figs.~\ref{fig:time_ic}-\ref{fig:time_tv} ). This massive scalability of \gc is a result of low storage overhead (only the graph and GCN and Q-learning parameters; detailed Space complexity provided in App.~\ref{app:complexity}) and relying on just forwarded passes through GCN and $Q$-learning. % three key design choices. First, other than storing the graph and a small number of parameters of the neural model (analysis in App~\ref{app:neuralparameters}), there is no additional storage overhead in \gc. %In contrast, IMM needs to construct and store reverse reachability sets, which does not scale even on Orkut. 
 %Second, instead of expensive path enumerations to estimate spread, \gc predicts the node quality, which is significantly cheaper. Finally, using the optimization strategies in \S~\ref{sec:optimizations}, $Q$-learning is performed on a significantly smaller set of \emph{promising} nodes. (See Fig.~\ref{fig:vb} in Supplementary).
 


\textbf{Performance on YT and Stack:} Since IMM crashes on Orkut, TW, and FS, we compare the quality of \gc with IMM on YT and Stack. Table~\ref{tab:sd} reports the results in terms of \emph{spread difference}, where $\text{Spread Difference}=\frac{f(S_{IMM})-f(S_{\gc})}{f(S_{IMM})}\times 100$.   $S_{IMM}$ and $S_{\gc}$ are answer sets computed by IMM and \gc respectively. A negative spread difference indicates better performance by \gc. The expected spread of a given set of nodes $S$, i.e. $f(S)$, is computed by taking the average spread across $10,000$ Monte Carlo simulations. %We repeat each experiment $5$ times by training on different subgraph samples of YT (CO and TV) and Stack (LND).

 Table~\ref{tab:sd} shows that the expected spread obtained by both techniques are extremely close. %While \gc is marginally better in YT-TV and Stack-LND, IMM is slightly superior in quality on the rest of the scenarios. %Second, although \gc is trained with solution sets of IMM, the fact that it is able to supersede IMM's performance on unseen test datasets indicates that $Q$-learning is able to learn a generalized policy.
%As visible, the spread difference is $\approx 1\%$ in YT-TV and $\approx 0\%$  in all of the remaining setups. 
 The true impact of \gc is realized when Table~\ref{tab:sd} is considered in conjunction with Figs.~\ref{fig:speedup_yt}-\ref{fig:speedup_st}, which shows \gc is $30$ to $160$ times faster than IMM. In this plot, speed-up is measured as $\frac{time_{IMM}}{time_{\gc}}$ where $time_{IMM}$ and $time_{\gc}$ are the running times of IMM and \gc respectively. 




%Overall, these results imply that: {\bf (1)} \gc matches the state-of-the-art technique for IM in spread quality, while being orders of magnitude faster. {\bf (2)} Instead of solving combinatorial problems repeatedly from scratch in dynamic networks, \gc provides an efficient and effective alternative approach, where we learn from past, low-volume data and predict on current, high volume data.



==> 6_prevwork.tex <==
%\clearpage
\section{Previous Work}
%Many combinatorial graph problems lead to NP-hardness \cite{karp1972reducibility}.There are classical NP-hard problems on graphs such as Minimum Vertex Cover, Minimum Set Cover, Travelling Salesman Problem (TSP); as well as other important combinatorial problems with many applications. Examples include finding top influential nodes \cite{kempe2003maximizing}, maximizing centrality of nodes \cite{yoshida2014almost}, and optimizing networks \cite{medya2018noticeable,dilkina2011}.

There has been recent interest in solving graph combinatorial problems with neural networks and reinforcement learning \cite{bello2016neural,dai2017learning}. Learning-based approaches are useful in producing good empirical results for NP-hard problems. The methods proposed in \cite{bello2016neural} are generic and do not explore structural properties of graphs, and use sample-inefficient policy gradient methods. Our work is very relevant to the work by Dai et al. \cite{dai2017learning}. They have investigated the same problem with a network embedding approach combined with a reinforcement learning technique. The main difference in this paper is the supervised part in our framework. Instead of an end-to-end learning, we use GCN to filter out the potential nodes in the solution. The second major difference is that our method is scalable and we apply it to the very popular data mining problem, Influence Maximization. 

The same problem has been studied by Li et al. \cite{li2018combinatorial} via a supervised approach using GCN. However, their technique involves multiple calls of GCN after selection of one element in the solution set. Their method also has an exploration part in a brute-force manner. Unsurprisingly besides independent set problem, this method is not scalable in other problems (e.g. Influence Maximization). Our method applies GCN once and finds the potential solution. Unlike in the previous one, we also apply reinforcement learning to construct our solution. Experimental results show that our method is more applicable to important problems such as Influence Maximization.




%Silver et al.[34,% used reinforcement learning to learn strategies for the game Go that achieved unprecedented
%results.  Vinyals et al.
%[37]
%developed a new neural network architecture called a pointer network,
%and applied it to small-scale planar Travelling Salesman Problem (TSP) instances with %up to 50
%nodes. 

